BloomCoreset: Fast Coreset Sampling using Bloom Filters for Fine-Grained Self-Supervised Learning

The success of deep learning in supervised fine-grained recognition for domain-specific tasks relies heavily on expert annotations. The Open-Set for fine-grained Self-Supervised Learning (SSL) problem aims to enhance performance on downstream tasks by strategically sampling a subset of images (the Core-Set) from a large pool of unlabeled data (the Open-Set). In this paper, we propose a novel method, BloomCoreset, that significantly reduces sampling time from Open-Set while preserving the quality of samples in the coreset. To achieve this, we utilize Bloom filters as an innovative hashing mechanism to store both low- and high-level features of the fine-grained dataset, as captured by Open-CLIP, in a space-efficient manner that enables rapid retrieval of the coreset from the Open-Set. To show the effectiveness of the sampled coreset, we integrate the proposed method into the state-of-the-art fine-grained SSL framework, SimCore [1]. The proposed algorithm drastically outperforms the sampling strategy of the baseline in SimCore [1] with a $98.5\%$ reduction in sampling time with a mere $0.83\%$ average trade-off in accuracy calculated across $11$ downstream datasets.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sections/1.introduction_bkp.tex <==
\section{Introduction}
\label{sec:intro}

The advent of deep neural networks (DNNs) has introduced a new era in a variety of domains, notably in image recognition \cite{he2016deep}, semantic segmentation \cite{badrinarayanan2017segnet,long2015fully}, image synthesis \cite{chen2017photographic,rombach2022high}, and 3D analysis \cite{qi2017pointnet,fischer2021stickypillars}. Their effectiveness, often surpassing human-level performance in computer vision, speech recognition, and natural language processing, is largely attributable to extensive training on voluminous labeled datasets. However, this dependency on large-scale annotated data presents a considerable bottleneck, especially in specialized medical imaging fields where expert annotations are crucial. Drawing inspiration from \cite{kim2023coreset}, the proposed work focuses on developing a sampling algorithm for constructing a subset of data in domain-specific tasks by leveraging an Open-Set, particularly where differentiation between subtly distinct images is essential. Our study operates under the realistic constraint of limited labeled samples for a fine-grained, domain-specific dataset. It proposes leveraging unlabeled data through self-supervised learning techniques.

\begin{table}[!t]
\caption{\textbf{Sampling time.} We have compared the coreset sampling time between SimCore \cite{kim2023coreset} and our BloomSSL method. The proposed method is better than the SimCore in order-of-magnitude time. This is due to the pre-training of the self-supervised method required in the case of SimCore to sample the closest image from Open-Set. Here, the Open-Set is imagenet1k \cite{deng2009imagenet}, and time is computed on two Rtx 3090 GPU.}
\resizebox{\linewidth}{!}{
\def\arraystretch{1}
\begin{tabular}{lcccc}
\hline
         & \multicolumn{2}{c}{SimCore ~\protect\cite{kim2023coreset}}                                                                                                                       & \multicolumn{2}{c}{BloomSSL (Ours)}                                                                                                                    \\ \cline{2-5} 
         & \begin{tabular}[c]{@{}c@{}}Preprocessing\\ (Sampling)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training \\ (Coreset+\\ Downstream )\end{tabular} & \begin{tabular}[c]{@{}c@{}}Preprocessing\\ (Sampling)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training\\ (Coreset+\\ Downstream)\end{tabular} \\ \hline
Open-Set & $\sim$23h 0m                                                       & $\sim$25h 0m                                                                 & \textbf{$\sim$0h 20m}                                                       & $\sim$25h 0m                                                               \\ \hline
\end{tabular}}
\label{table:time}
% \end{wraptable}
\end{table}

\textbf{Self Supervised Learning:}
Recent advancements in self-supervised learning (SSL) \cite{grill2020bootstrap,caron2021emerging} have paved the way for learning data representations without reliance on annotations, effectively improving the results of subsequent downstream tasks. Unlike unsupervised representation learning \cite{gidaris2018unsupervised,zhang2016colorful}, where the handcrafted pretext tasks are difficult to generalize and scale,
contrastive learning \cite{chen2020simple,oord2018representation} focuses on creating positive pairs by image augmentation and using distinct images as negative samples. SSL benefits from the abundance of unlabeled data obtainable through web crawling \cite{goyal2021self} and remove the dependence on labeling, which is particularly advantageous. Our study's focus is on the Open-Set Self-Supervised Learning (OpenSSL) task, as introduced by \cite{kim2023coreset}, where we utilize the large-scale open-sets for aiding the SSL pretraining using the specific fine-grained target datasets.

\textbf{Motivation for Coreset:}
\cite{ericsson2021well} highlights a correlation between the performance of self-supervised learned representations on downstream tasks and the similarity of the pretraining and fine-tuning datasets. This distribution mismatch issue is particularly pronounced in OpenSSL due to irrelevant instances in the Open-Set, which can impede the learning of useful representations. Our study inspired by  \cite{kim2023coreset} tackles distribution mismatch by curating a coreset from the Open-Set that aligns semantically with limited fine-grained labeled samples, enhancing SSL efficacy on downstream tasks. This focused approach outperforms the use of the entire Open-Set, as substantiated by the results in Table \ref{table:simclrall}, underscoring the benefits of tailored data curation in SSL.

% \begin{wraptable}{r}{6.9cm}

\textbf{Coreset Sampling.}
A coreset is a subset of an Open-Set that shares semantic similarities with the downstream dataset. The study by \cite{kim2023coreset} highlights the performance benefits of integrating a coreset with the downstream dataset $X$, compared to either the entire Open-Set $(X+OS)$ or a randomly sampled subset $(X+OS_{rand})$. However, existing sampling algorithms, such as those discussed in \cite{kim2023coreset,sener2017active,wei2015submodularity}, 
exhibit substantial computational latency, rendering them impractical as off-the-shelf solutions and do not take into consideration the distribution discrepancies in the Open-Set. Our research proposes BloomSSL to address these gaps. This novel strategy drastically improves the coreset sampling speed while preserving competitive performance compared to the state-of-the-art baseline.

% Table \ref{table:time} shows our sampling speed outperforms the state-of-the-art sampling strategy by $98.5\%$ reduction in sampling time with a mere $0.83\%$ average trade-off in accuracy calculated across $11$ datasets. Alongside addressing the limitations in \cite{kim2023coreset}, our work also explores the distribution discrepancy in the data in the context of long-tailed datasets. This analysis is crucial as it sheds light on the inherent challenges posed by skewed data distributions, which are often overlooked yet significantly impact SSL model performance and generalization.

The primary contributions of this work are given below.
\begin{enumerate}

\begin{figure}[!t]
  \centering
  \includegraphics[width=1.0\linewidth]{images/pipeline.pdf}
  \caption{\textbf{BloomSSL Framework.} The figure illustrates the envisioned workflow for addressing an OpenSSL problem. Leveraging the pre-trained OpenCLIP model by ~\protect\cite{cherti2023reproducible}, we extracted image features (hash codes) from both domain-specific and open-set image pools. Subsequently, these features undergo processing through the innovative BloomSSL algorithm, designed to generate a coreset from the open-set image pool. The resulting coreset and domain-specific data were utilized to train our self-supervised methodology.}  
  \label{fig:block_diagram}
\end{figure}

\item \textbf{Faster Samples Retrieval} - We employ a probabilistic data structure Counting Bloom Filter/Bloom Filter \cite{fan2000summary,bloom1970space} to significantly expedite the retrieval of semantically similar images from large Open-Sets as shown in Fig.\ref{fig:block_diagram} and Fig.\ref{fig:samplingdiag}.

\item \textbf{Performance} - Our work demonstrates competitive performance over existing sampling strategies across a wide range of fine-grained datasets (Table \ref{table:simclrall}) and Open-Sets (Fig.\ref{fig:compalldataset}), as evidenced by extensive experimental evaluations.
\end{enumerate}

==> sections/2.method_bkp.tex <==
\section{Method}
\label{sec:method}

In this work, we proposed a fast coreset sampling method that acts as a module for Open-Set self-supervised learning, as shown in Fig.\ref{fig:block_diagram}. The proposed modular framework consists of two phases: 1) Generating features for both downstream dataset and Open-Set using pre-trained Open-CLIP \cite{cherti2023reproducible}. These generated features are used to build the coreset with the help of bloom filters and top-$k$ filtering. The proposed sampling method improves the sampling time by orders of magnitude. 2) Using the sampled coreset and downstream data to train a self-supervised method, which later can be utilized for domain-specific tasks.

\begin{figure}[!t]
\centering
 \includegraphics[width=0.9\linewidth]{images/algorithmflowchart.pdf}
\caption{\textbf{Bloom Filter and Sampling.} The domain-specific features are used to build the counting bloom filter (CBF). Following this, a membership test is performed to sample images from Open-Set, which are similar to domain-specific images. After sampling domain-specific similar images from the Open-Set, the inner product is calculated, and further filtering is applied to select the best subset from sampled open-set images. In section \ref{subsec:coresetexpalin}, we have given a complete overview of the sampling method.}
\label{fig:samplingdiag}
\end{figure}

\subsection{Background}
\label{sec:background}

In alignment with the paradigm established by \cite{kim2023coreset}, our methodology entails the generation of augmented pairs 
$(x_{i}^{t_{1}}, x_{i}^{t_{2}})$ from the given data corpus $\mathcal{X}=\left\{x_{i}\right\}_{i=1}^{N}$. An encoder network $E_{\theta}$ is trained on a random batch from training data $(\mathcal{X_{B}})$ with the objective of the minimization of the contrastive loss as proposed in \cite{chen2020simple} by projecting the positive pair $(x_{i}^{t_{1}}, x_{i}^{t_{2}})$ close in the representation space and contrasting it from all the negative pairs $\{(x_{j}^{t_{1}}, x_{j}^{t_{2}}) | j \neq i, (i,j) \in \{1, 2, ..., N_{B}\} \}$.

\begin{align}
    &\mathcal{L}_{c} = \underset{x_{i} \in \mathcal{X_{B}}, x_{j} \in \mathcal{X_{B}}}{\mathbb{E}} \Bigg[-log\frac{exp(sim(z_{i}, z_{j})/\tau)}{\sum\limits_{k=1}^{2N_{B}}\mathbbm{1}_{[k \neq i]} exp(sim(z_{i}, z_{k})/\tau)} \Bigg] \notag \\
    \label{eqn:1}
\end{align}

Here, $L_{c}$ is the contrastive loss, $z = E_{\theta}\left(x^{t}\right)$ denotes the representation from encoder $E$ parameterized over $\theta$ which are the learnable parameters. $N_{B}$ is the number of samples in the image batch and $(t_{1}, t_{2})$ are the pair of transformations from transformation space $\mathcal{T}$.

\textit{In the context of the OpenSSL problem, our objective is to sample such data from Open-Set ($\mathcal{U}$) whose inclusion in the downstream dataset ($\mathcal{X}$) improves the performance of representation learning of the SSL method.}

\subsection{Coreset Sampling from Open-Set}
\label{subsec:coresetexpalin}

The work by \cite{kim2023coreset} first trains a self-supervised method on the downstream dataset and later uses it to sample the closest images from Open-Set. However, this process is inherently time and resource-intensive, especially given the recent trend of employing multi-modal SSL methods trained on extensive datasets, often encompassing millions of data points. Recognizing the substantial computational expense associated with this traditional method, our work pivots towards a more efficient paradigm.

In the last few years, billions of data \cite{schuhmann2022laionb} has been used to train multi-modal self-supervised methods \cite{Radford2021LearningTV,cherti2023reproducible}, and their pre-trained weights are available for fine-tuning or testing.  In this work, we have proposed a sampling algorithm (BloomCoreset) that reduces the time needed to sample data from Open-Set. We have used a pre-trained Open-CLIP \cite{cherti2023reproducible} as a feature extractor backbone for both downstream and Open-Set data, as shown in Fig.\ref{fig:block_diagram}. 

% \begin{wrapfigure}{r}{8cm}
\begin{figure}[!t]
\begin{minipage}{\linewidth}
\removelatexerror% Nullify \@latex@error
\begin{algorithm}[H]
\DontPrintSemicolon  
  \KwInput{$E_{\theta}$: pre-trained open clip image encoder}
  \KwInput{$\mathcal{U}$: all the images in open-set}
  \KwInput{$\mathcal{X}$: all the images in downstream dataset}
  \KwInput{$CBloomFilter()$: method that returns object of CBF, $\mathcal{B}$: coreset budget}
  % \tcc{size of downstream dataset}
  initialize $N_{\mathcal{X}} \xleftarrow{} |\mathcal{X}|$, $h_{size} \xleftarrow{} 10000 \times (N_{\mathcal{X}}/3500) $ \\
  % \tcc{size of CBF bit array}
   initialize $c_{size} \xleftarrow{} 32 $, $feat_{\mathcal{X}} \xleftarrow{} \emptyset$\\
   % \tcc{downstream and open-set clip features}
  initialize $feat_{\mathcal{U}} \xleftarrow{}  \emptyset$, $member_{\mathcal{U}} \xleftarrow{}  \emptyset$ \\
  % \tcc{store matched images from open-set}
  % initialize $coreset_{idx} \xleftarrow{} \emptyset$, $coreset \xleftarrow{}  \emptyset$ \\
  % \tcc{false positive rate for CBF}
  % \tcc{counter's bit length for CBF}
  $cbloom \xleftarrow{} CBloomFilter(h_{size}, c_{size})$ \\
  \tcc{Creating counting bloom filter (CBF)}
  \For{$I_{\mathcal{X}} \in \mathcal{\mathcal{X}}$}
   {
        $z \xleftarrow{} E_{\theta}(I_{\mathcal{X}})$ \tcp*{ $z \in \mathbb{R}^{512}$}
        $feat_{\mathcal{X}}.append(z)$ \\
        $bin_{z} \xleftarrow{} where(z < 0, 0, 1)$ \\
        $cbloom.update(bin_{z})$ \\
   }
   \tcc{Sampling from the open-set using CBF}
   \For{$I_{\mathcal{U}} \in \mathcal{U}$}
   {
        $z \xleftarrow{} E_{\theta}(I_{\mathcal{U}})$ \tcp*{ $z \in \mathbb{R}^{512}$}
        $feat_{\mathcal{U}}.append(z)$ \\
        $bin_{z} \xleftarrow{} where(z < 0, 0, 1)$ \\
        \If{$cbloom.check(bin_{z})$}
        {
            $member_{\mathcal{U}}.append(z)$
        }
   }
   \tcc{Refining the images from $member_{\mathcal{U}}$}
   % \tcc{size of matched images list}
   $N_{M} \xleftarrow{} |member_{\mathcal{U}}|$ \\
   % \tcc{$simscore \in \mathbb{R}^{N_{D} \times N_{M}}$}
   $simscore \xleftarrow{} feat_{\mathcal{X}} \times member_{\mathcal{U}}.T$ \tcp*{$\mathbb{R}^{N_{\mathcal{X}} \times N_{M}}$}
   % $simscore \xleftarrow{} Sort.descending(simscore)$ \\
   % \For{$i \in range(N_{D})$}
   % {
   %      $coreset_{idx} \xleftarrow{} TopK\_Index(simscore[i, :])$ \\
   % }
   % $coreset_{idx} \xleftarrow{} Unique(coreset_{idx})$ \\
   % % \tcc{select images from index}
   % $coreset \xleftarrow{} X[coreset_{idx}]$ \\
   $coreset \xleftarrow{} Filter(simscore, \mathcal{\mathcal{U}}, \mathcal{B})$ \\
   \KwOutput{$coreset$}
\caption{Sampling image subset (coreset) from the open-set images}
\label{algo:coresetsampling}
\end{algorithm}
\end{minipage}
\end{figure}
% \vspace{-5pt}
% \end{wrapfigure}

To sample images closer in the feature space of the downstream dataset from Open-Set, we proposed an innovative framework using Bloom Filters \cite{bloom1970space} as a hashing mechanism. The bloom filters are a probabilistic data structure used in membership testing to achieve zero false positives. Building on this idea, we used Open-CLIP features extracted from downstream datasets to create a bloom filter data structure, and in the backend of the bloom filter, the murmurhash3 \cite{murmurhash3} hash function $(F^{cbf})$ is used for building the hash table. We have used ten different variations of murmurhash3 $(F_{i}^{cbf})$ to build a bloom filter. For sampling the coreset, we performed membership testing on the Open-CLIP features extracted from Open-Set images. 

The time complexity for adding an item or checking membership in a Bloom filter is $O(h)$, where $h$ is the number of hash functions used. This means that regardless of the number of items in the filter, the time it takes to perform these operations remains constant and is independent of the data size. Additionally, membership testing requires a single access to the data structure, significantly reducing the memory access time. 
Thus, harnessing a pre-trained model trained on billions of data points alongside an efficient data structure like the bloom filter helps obtain robust feature representation at a fraction of the time taken by \cite{kim2023coreset}.

% \begin{figure}[!t]
% \centering
% % \resizebox{\textwidth}{!}{
% % \def\arraystretch{2}
% \begin{tabular}{cc}
%     \includegraphics[width=.4\linewidth]{images/plots/topk_plot_imagenet_pets.pdf}      &    \includegraphics[width=.4\linewidth]{images/plots/topk_plot_imagenet_food11.pdf}    \\
%     \includegraphics[width=.4\linewidth]{images/plots/topk_images_imagenet_pets_compressed.pdf}      &  \includegraphics[width=.4\linewidth]{images/plots/topk_images_imagenet_food11_compressed.pdf}  \\
% (a) Pets & (b) Food \\
% \end{tabular}
% % }
% \caption{\textbf{Coreset Samples.} Visualization of sampled coreset from Open-Set with the proposed bloom filter-based method. The histogram plot shows the top-$20$ sample frequencies across different downstream datasets. This shows the sampled coreset can capture data distribution of downstream datasets with semantically closed images.}
% \label{fig:sampledimages}
% \end{figure}

\begin{figure}[!t]
    \begin{minipage}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/plots/comparison.pdf}
        \captionof{figure}{\textbf{Other open-set.} Comparison across different Open-Sets, the learned representation from the coreset sampled using the proposed method shows competitive performance to the baseline and, in some cases, outperforms the baseline.}
        \label{fig:compalldataset}
    \end{minipage}
    % \hspace{0.05cm}
    % \begin{minipage}[b]{0.49\linewidth}
    %     \centering
    %     % \vspace{2cm}
    %     \resizebox{\linewidth}{!}{\begin{tabular}{ccccc}
    %         & \LARGE{Clip Downstream} & \LARGE{Clip Coreset} & \LARGE{Pre-trained Downstream} & \LARGE{Pre-trained Coreset} \\
    %        \rotatebox[origin=c]{90}{\huge{(a) Aircraft}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreamaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreamaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetaircraft.png}      \\
    %         \rotatebox[origin=c]{90}{\huge{(b) Pets}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreampets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetpets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreampets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetpets.png}      \\
    %         \rotatebox[origin=c]{90}{\huge{(c) Food}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreamfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreamfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetfood11.png}
    %     \end{tabular}}
    %     % \vspace{0.35cm}
    %     \captionof{figure}{\textbf{Feature distribution.} Show representation space of Open-CLIP ~\protect\cite{cherti2023reproducible}. We have used Gaussian kernel density estimation ~\protect\cite{wang2020understanding} to show the feature distribution of downstream dataset samples and coreset samples across the unit ring.}
    %     \label{fig:featdist}
    % \end{minipage}
\end{figure}

Interestingly, using the coreset generated by bloom filters and the downstream dataset doesn't improve the representation learning performance much, as shown in \ref{table:randombloom}. This is because false positive samples are present in the coreset due to the properties of the bloom filters. The bloom filters have zero-false negative, which causes an increase in false positive samples. We proposed a top-$k$ filtering method over the sampled coreset to handle this issue. In the top-$k$ method, we compute the cosine similarity score between the filtered and downstream samples. The calculated similarity score is then used to retrieve samples from filtered Open-Set closer to the downstream dataset (see Algorithm \ref{algo:coresetsampling}). The complete sampling pipeline is illustrated in Fig.\ref{fig:samplingdiag}, where $N_{\mathcal{X}}$ is the number of samples in the downstream dataset, $N_{\mathcal{U}}$ is the number of samples in Open-Set, $N_{M}$ is the number of filtered samples from Open-Set after membership testing using counting bloom filter and $N_{F}$ is the final coreset size after applying top-$k$ filtering.

% \subsection{Frequency-Aware SSL}

% Once we have the coreset sampled from Open-Set, we further study the possibility of long-tailed distribution being present in the union of downstream and coreset data. Different strategies have been proposed to handle long-tailed distribution data in the previous works \cite{cui2019class}. One such strategy is re-sampling, where we can either populate the dataset set by augmenting the existing data or discard some data samples so each class has an equal number of images. The problem with these approaches is that they either overfit the model due to over-sampling or can lead to degenerated representation due to under-sampling \cite{cui2019class}. Overcoming this problem \cite{cui2019class} proposes a strategy to re-weight the classes based on the sample's frequency, which has also been used in the proposed work. 

% The imbalance factor of the dataset can be handled by considering the frequency of samples, where the class with the least number of samples has high weights in loss function compared to the classes in the dataset with a high number of samples. So, the weighting factor is introduced in the Equation \ref{eqn:1} as follows:

% \begin{align}
%     &\mathcal{L}_{contra} = \mathbb{E}_{x_{i} \sim \mathcal{X}} \Bigg[- w_{i} log\frac{exp(sim(z_{i}, z_{j})/\tau)}{\sum\limits_{k=1}^{2N}\mathbbm{1}_{[k \neq i]} exp(sim(z_{i}, z_{k})/\tau)} \Bigg] \notag \\
%     &\text{where,} \quad w_{i} = \frac{(1-\beta)}{1-\beta^{c_{i}}}
%     \label{eqn:2}
% \end{align}

% In Equation \ref{eqn:2}, $w_{i}$ is the weight associated with each class $i$, $c_{i}$ is the number of images in the $i$th class, and $\beta$ is the re-weighting term. Following \cite{cui2019class}, "$\beta=0$ implies no class-based re-weighting and $\beta \xrightarrow{} 1$ implies re-weighting by inverse class frequency". In the proposed work, we have used counting bloom filter \cite{5374398} to get the frequency of sampled coreset from Open-Set. Table \ref{table:simclrablation} shows the performance across eleven different datasets when the SSL method is trained using weighted frequency loss.

\begin{table*}[!t]
\centering
\caption{Comparison of representation learned using the coreset sampled using our proposed method and the baseline ~\protect\cite{kim2023coreset} method on the classification accuracy. The coreset generated using the proposed method shows competitive performance in many downstream datasets and outperformed the previous accuracy for some downstream datasets. This can be seen as a trade-off between sample quality and speed.}
\resizebox{\linewidth}{!}{
\def\arraystretch{1.2}%
\begin{tabular}{lcccccccccccc} \hline
\multicolumn{1}{c}{}  &     & \multicolumn{11}{c}{Target dataset (X) and its number of samples}                               \\
\multicolumn{1}{c}{}  &     & Aircraft & Cars  & Pet   & Birds & Dogs  & Flowers & Action & Indoor & Textures & Faces & Food  \\ 
Pretrain              & p   & $6667$     & $8144$  & $3680$  & $5990$  & $12000$ & $2040$    & $4000$   & $5360$   & $3760$     & $4263$  & $13296$ \\ \hline
$\mathcal{X}$                     & -   & $46.56$    & $55.42$ & $59.23$ & $29.27$ & $49.88$ & $80.14$   & $43.76$  & $54.10$  & $58.78$    & $56.63$ & $87.99$ \\
$\mathcal{X}+OS$                  & -   & $39.88$    & $42.92$ & $68.22$ & $32.88$ & $50.42$ & $\underline{85.34}$   & $\textbf{60.61}$  & $\underline{63.66}$  & $\textbf{67.98}$    & $52.76$ & $85.90$ \\ 
$\mathcal{X}+OS_{rand}$         & 1\% & $48.24$    & $49.26$ & $64.27$ & $31.90$ &$ 49.62$ & $83.17$   & $47.25$  & $55.37$  & $61.33$    & $\underline{57.37}$ & $88.08$ \\ \hline
$\mathcal{X}+OS_{SimCore}$  ~\protect\cite{kim2023coreset}    & 1\% & $\textbf{50.79}$    & $\textbf{57.90}$ & $\textbf{76.90}$ & $\textbf{36.94}$ & $\textbf{59.83}$ & $\textbf{86.70}$   & $52.98$  & $59.18$  & $63.40$    & $\textbf{58.85}$ & $\underline{89.78}$ \\
$\mathcal{X}+OS_{BloomSSL}$ (Ours) & 1\% &    $\underline{49.34}$      &   $\underline{52.08}$    &   $\underline{76.20}$    &  $\underline{35.96}$    &   $\underline{54.43}$    &    $84.56$     &   $\underline{56.76}$     &    $\textbf{63.66}$    &     $\underline{65.11}$     &   $55.72$    &    $\textbf{90.20}$   \\ \hline

\end{tabular}}
\label{table:simclrall}
\end{table*}

==> sections/3.experiment_bkp.tex <==
\section{Experiments}
\label{sec:experiments}

% This section discusses the experimental setup followed throughout the study. The first part of the section focuses on evaluating the representations learned using the proposed BloomSSL method and its comparison with the baseline method \cite{kim2023coreset}. In the second part of the experiment, we focused on the ablation study that includes different sampling strategies and feature extractor backbones.

\subsection{Network Training and Datasets}

We have used the eleven downstream datasets and three Open-Set for evaluation and comparison: Aircraft \cite{maji2013fine}, Cars \cite{krause20133d}, Pet \cite{parkhi2012cats}, Birds \cite{welinder2010caltech}, Dogs \cite{khosla2011novel}, Flowers \cite{nilsback2008automated}, Action \cite{yao2011human}, Indoor \cite{quattoni2009recognizing}, Textures \cite{cimpoi2014describing}, Faces \cite{lee2020maskgan}, Food \cite{singla2016food}, Imagenet1k \cite{deng2009imagenet}, MS COCO \cite{lin2014microsoft}, and iNaturalist 2021-mini \cite{van2018inaturalist}.

For the self-supervised learning backbone, we used SimCLR \cite{chen2020simple} with ResNet50. We have trained the network on two GPUs with a batch size of $256$. For a fair comparison, we have kept all the experimental setups similar to the SimCore \cite{kim2023coreset} and re-run most of the experiments of SimCore with batch size $256$ on two GPUs. In all the experiments, including SimCore and ours, we kept a threshold on the size of the coresets as $1\%$, i.e., we consider only $1\%$ of sampled coreset data for training the SSL method.
% The output feature size of the Open-CLIP \cite{cherti2023reproducible} method is $512$.

\subsection{Analysis of Sampling Method}

Using the bloom filters, we sample the coreset from Imagenet1k \cite{deng2009imagenet} for each downstream dataset. With the sampled coreset and downstream data, we train the SimCLR \cite{chen2020simple} network. To compare with the baseline, we follow the linear evaluation strategy, using the pre-trained SimCLR network as a feature extractor and training an image classification network in a supervised setting.

% % \begin{wraptable}{!r}{6.3cm}
% \begin{table}
% \centering
% \caption{\textbf{Long-tail.} Shows the performance on long-tailed dataset. We have kept the imbalance ratio for the downstream dataset as $\rho = 0.1$ following the work ~\protect\cite{tang2020long}.}
% \resizebox{0.45\textwidth}{!}{
% \def\arraystretch{1.2}
% \begin{tabular}{llll}
% \hline
%                    &     & Flowers & Pets    \\
% Pretrain           & p   &    2040     &    3680     \\ \hline
% $\mathcal{X}+OS_{SimCore}$ ~\protect\cite{kim2023coreset} & 1\% & $\textbf{57.44}$ & $\textbf{65.71}$ \\
% $\mathcal{X}+OS_{BloomSSL}$ (Ours) & 1\% & $56.69$ & $63.48$ \\ \hline
% \end{tabular}}
% \label{table:longtail}
% \vspace{-5pt}
% % \end{wraptable}
% \end{table}


We have used a variation of the bloom filter known as counting bloom filter \cite{5374398}. Counting bloom filters store a count of how many times a particular hash location is accessed while storing the information. We used this property to store the frequency of each sample in the downstream dataset and the sampled coreset. The coreset sampling procedure is mentioned in Fig.\ref{fig:samplingdiag}.

\begin{table}[t]
\centering
\caption{\textbf{Random Bloom.} Quantitative results of using samples from a bloom filter without applying the proposed post-filtering approach degrade the performance.}
\begin{tabular}{lccccc}\hline
         &     & \multicolumn{4}{c}{Target Dataset (X)} \\
         &     & Pet                & Flowers              & Textures    & Action         \\
Pretrain & p   & $3680$               & $2040$                 & $3760$       & 4000          \\ \hline
$\mathcal{X}$ + $OS_{BloomSamples}$   & $1\%$ & $67.56$              & $82.16$                & $62.66$   &  $50.89$    \\ \hline
$\mathcal{X}$ + $OS_{base}$   & $1\%$ & $76.20$              & $84.56$                & $65.11$        &  $\textbf{56.76}$      \\
$\mathcal{X}$ + $OS_{sum}$   & $1\%$ & $76.45$              & $\textbf{85.09}$                & $\textbf{66.49}$  &      $53.89$        \\
$\mathcal{X}$ + $OS_{max}$   & $1\%$ & $\textbf{76.78}$              & $84.48$                & $65.11$     & $55.55$          \\
\hline
\end{tabular}
\label{table:randombloom}
\end{table}

\textbf{Sampling and Classification.} In Table \ref{table:simclrall}, we have shown the comparison between the coreset quality sampled using SimCore \cite{kim2023coreset} and BloomSSL method (ours). Our proposed method shows competitive performance in representation learning, and for some downstream datasets, the representation learned using the sampled coreset from our method outperformed the baseline method. This also shows the trade-off between coreset sampling speed and quality. Using the conventional sampling method can give fewer false positive samples but consume a considerable amount of time in training and sampling. Still, with BloomSSL, we can improve the sampling time with a small loss of accuracy. In Table \ref{table:time}, we have shown a comparison of time required for BloomSSL (ours) and SimCore \cite{kim2023coreset}. As shown in Table.\ref{table:randombloom}, using samples obtained using bloom filter without applying top-$k$ strategy shows degraded performance.

 % method for sampling coreset from Open-Sets and training the SSL method for representation learning on combined coreset with downstream dataset.
% \begin{table*}[!t]
% \centering
% \caption{\textbf{Filtering Ablation.} Shows the result of different filtering methods. After computing the cosine similarity matrix, we study different approaches to sample top-$k$ images. These include sorting the scores (base), taking sums, and taking maxes. In the last row, we have shown the performance of representation learning when the network is trained using the frequency count of each image, which we obtained using a counting bloom filter.}
% \resizebox{\linewidth}{!}{
% \def\arraystretch{1.2}
% \begin{tabular}{lcccccccccccc} \hline
% \multicolumn{1}{c}{}  &     & \multicolumn{11}{c}{Target dataset (X) and its number of samples}                               \\
% \multicolumn{1}{c}{}  &     & Aircraft & Cars  & Pet   & Birds & Dogs  & Flowers & Action & Indoor & Textures & Faces & Food  \\ 
% Pretrain              & p   & $6667$     & $8144$  & $3680$  & $5990$  & $12000$ & $2040$    & $4000$   & $5360$   & $3760$     & $4263$  & $13296$ \\ \hline
% $\mathcal{X}+OS_{Bloom}$ (Base) & 1\% &    $49.34$      &   $52.08$    &   $76.20$    &  $35.96$    &   $54.43$    &    $84.56$     &   $\textbf{56.76}$     &    $63.66$    &     $65.11$     &   $\textbf{55.72}$    &    $90.20$   \\
% $\mathcal{X}+OS_{Bloom}$ (Sum) & 1\% &    $\textbf{51.13}$      &   $\textbf{53.42}$    &   $76.45$    &   $\textbf{36.70}$    &   $53.89$    &    $85.09$     &   $53.89$     &    $61.73$    &     $\textbf{66.49}$     &   $54.89$    &    $\textbf{91.32}$   \\
% $\mathcal{X}+OS_{Bloom}$ (Max) & 1\% &    $49.86$      &   $52.67$    &   $76.78$    &  $35.92$    &   $54.21$    &    $84.48$     &   $55.55$     &    $63.73$    &     $65.11$     &   $55.56$    &    $89.78$   \\\hline
% $\mathcal{X}+OS_{Bloom}$ (Frequency Loss) & 1\% &    $48.86$      &   $51.78$    &   $\textbf{77.23}$    &  $33.36$    &   $\textbf{55.82}$    &    $\textbf{85.46}$     &   $54.97$     &    $\textbf{64.20}$    &     $63.56$     &   $54.30$    &    $90.32$   \\\hline
% \end{tabular}}
% \label{table:simclrablation}
% \end{table*}

% \textbf{Coreset Visualization.} Along with the quantitative analysis, we performed a qualitative analysis. In this, we computed the frequency of samples from each class in the Open-Set. We also visualized the random image from top-$20$ classes with the highest number of samples in the coreset. As in Fig.\ref{fig:sampledimages}, the top-$20$ classes in the coreset are semantically closest to the downstream datasets.

\begin{figure}[!t]
    % \begin{minipage}[b]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{images/plots/comparison.pdf}
    %     \captionof{figure}{\textbf{Other open-set.} Comparison across different Open-Sets, the learned representation from the coreset sampled using the proposed method shows competitive performance to the baseline and, in some cases, outperforms the baseline.}
    %     \label{fig:compalldataset}
    % \end{minipage}
    % \hspace{0.05cm}
    \begin{minipage}[b]{\linewidth}
        \centering
        % \vspace{2cm}
        \resizebox{\linewidth}{!}{\begin{tabular}{ccccc}
            & \LARGE{Clip Downstream} & \LARGE{Clip Coreset} & \LARGE{Pre-trained Downstream} & \LARGE{Pre-trained Coreset} \\
           \rotatebox[origin=c]{90}{\huge{(a) Aircraft}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreamaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreamaircraft.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetaircraft.png}      \\
            \rotatebox[origin=c]{90}{\huge{(b) Pets}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreampets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetpets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreampets.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetpets.png}      \\
            \rotatebox[origin=c]{90}{\huge{(c) Food}} & \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_downstreamfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/clip_densityplot_coresetfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_downstreamfood11.png}   &  \includegraphics[width=0.69\linewidth,valign=m]{images/density/pretrain_densityplot_coresetfood11.png}
        \end{tabular}}
        % \vspace{0.35cm}
        \captionof{figure}{\textbf{Feature distribution.} Show representation space of Open-CLIP ~\protect\cite{cherti2023reproducible}. We have used Gaussian kernel density estimation ~\protect\cite{wang2020understanding} to show the feature distribution of downstream dataset samples and coreset samples across the unit ring.}
        \label{fig:featdist}
    \end{minipage}
\end{figure}

\textbf{Various Open-Sets.} We have shown the performance of the BloomSSL method on a variety of Open-Sets other than imagenet1k, including MS COCO \cite{lin2014microsoft}, and iNaturalist 2021-mini \cite{van2018inaturalist}. Fig.\ref{fig:compalldataset} shows improvement in the performance across various downstream datasets using different Open-Sets in comparison to SimCore \cite{kim2023coreset} method. This shows the generalization property of the proposed coreset sampling method.

% \textbf{Long-tail Datasets.} We performed empirical studies using both SimCore \cite{kim2023coreset} and the proposed BloomSSL method to show the effectiveness of Open-SSL on long-tailed distribution datasets. We have used Flowers \cite{nilsback2008automated} and Pet \cite{parkhi2012cats} dataset for this study. To create a long-tail distribution, we follow the approach mentioned in work \cite{tang2020long} and keep the imbalance ratio $(\rho)=0.1$. This experiment aims to study the effect of the least frequent images/class in representation learning. Based on Table\ref{table:longtail}, there is a significant drop in classification accuracy in the case of long-tail distribution. Our proposed method shows competitive performance with SimCore because we are sampling images from Open-Set based on each image in the downstream dataset. This way, the sampled coreset handles the image imbalance problem. We have used the Equation \ref{eqn:2} i.e., frequency-based loss function for training the SSL method.

\textbf{Feature Density Map.} The density mapping in Fig.\ref{fig:featdist} shows that the pre-trained Open-CLIP method generates semantically rich features that span the entire unit ring \cite{wang2020understanding} due to a multi-modal training regime. This implies that if we do not use bloom filter and top-$k$ filtering, then the coreset we will obtain will consist of a diverse class of images from Open-Sets, which can lead to performance degradation. The pre-trained downstream plot in Fig.\ref{fig:featdist} can further verify this, which shows even after using a sampled coreset for training, the features distribution of pets concentrated at a certain location in the unit ring.

% \textbf{Ablation Studies.} We have performed several ablation studies on top-$k$ filtering method as shown in Table \ref{table:simclrablation}. In this study, we modified the filtering approach on the samples we got after the bloom filter membership test. Based on the experiments, we discovered that the coresets are sensitive to the filtering method. In max-based filtering, we take the maximum similarity score calculated between downstream and filtered Open-Set samples across the row and sort it according to the highest similarity score. Its equivalent filtered Open-Set index is selected as part of the coreset. For sum-based filtering, we have added the similarity score across the row, sorted it based on the summed score, and selected the filtered Open-Set index based on the highest score. We further performed one more ablation, in which we studied the effect using a frequency-based loss function for training the SSL method. Based on the ablation study, the proposed BloomSSL-based method performs better than all its counterparts.

==> sections/5.background.tex <==
\section{Background}
\label{sec:background}

In alignment with the paradigm established by \cite{kim2023coreset}, our methodology entails the generation of augmented pairs $(x_{i}^{t_{1}}, x_{i}^{t_{2}})$ from the given data corpus $\mathcal{X}=\left\{x_{i}\right\}_{i=1}^{N}$. An encoder network $E_{\theta}$ is trained on a random batch from training data $(\mathcal{X_{B}})$ with the objective of the minimization of the contrastive loss as proposed in \cite{chen2020simple} by projecting the positive pair $(x_{i}^{t_{1}}, x_{i}^{t_{2}})$ close in the representation space and contrasting it from all the negative pairs $\{(x_{j}^{t_{1}}, x_{j}^{t_{2}}) | j \neq i, (i,j) \in \{1, 2, ..., N_{B}\} \}$.

\begin{align}
    &\mathcal{L}_{c} = \underset{x_{i} \in \mathcal{X_{B}}, x_{j} \in \mathcal{X_{B}}}{\mathbb{E}} \Bigg[-log\frac{exp(sim(z_{i}, z_{j})/\tau)}{\sum\limits_{k=1}^{2N_{B}}\mathbbm{1}_{[k \neq i]} exp(sim(z_{i}, z_{k})/\tau)} \Bigg] \notag \\
    \label{eqn:1}
\end{align}

Here, $L_{c}$ is the contrastive loss, $z = E_{\theta}\left(x^{t}\right)$ denotes the representation from encoder $E$ parameterized over $\theta$ which are the learnable parameters. $N_{B}$ is the number of samples in the image batch and $(t_{1}, t_{2})$ are the pair of transformations from transformation space $\mathcal{T}$.

\textit{In the context of the OpenSSL problem, our objective is to sample such data from Open-Set ($\mathcal{U}$) whose inclusion in the downstream dataset ($\mathcal{X}$) improves the performance of representation learning of the fine-grained SSL method.}

